Modeling the measurement accuracy of pre-atmosphere velocities of meteoroids

Many existing optical meteor trajectory estimation methods use the approximation that the velocity of the meteor at the beginning of its luminous phase is equivalent to its velocity before atmospheric entry. Meteoroid kinetic energy loss prior to the luminous phase cannot be measured, but for some masses and entry geometries neglecting this loss may lead to non-negligible deceleration prior to thermal ablation. Using a numerical meteoroid ablation model, we simulate the kinematics of meteoroids beginning at 180 km with initial velocities ranging from 11 km/s to 71 km/s, and compare model velocities at the moment of detection to measurements. We validate the simulations by comparing the simulated luminous beginning heights with observed beginning heights of different populations of meteors detected with different optical systems. We find that most low-velocity meteoroids have a significant velocity difference of 100 m/s to 750 m/s (depending on meteoroid type, mass, and observation system). This systematic underestimate of meteoroid speeds also results in systematically lower semi-major axes for meteoroid orbits.

==> reviewers_comments_rev2.tex <==
> I am glad that my recommendations were taken into account. The manuscript 
> can be accepted after minor corrections listed below are done.


> I apologize that I overlooked that some formulations in the Introduction are
> not correct. Ceplecha (1987) did not assume that the measured velocity is 
> equal (after the correction to Earth rotation) to the no-atmospheric 
> velocity. He noted that velocity is computed from the measured length as a 
> function of time and recommended the fitting method of Pecina and Ceplecha 
> (1983, 1984). In this method, the pre-atmospheric velocity v_infinity is one 
> parameter of the fit. In practice v_infinity is computed at the height 150 km 
> (maybe this height is not mentioned in the papers). Of course, atmospheric 
> density profile must be postulated.
> Spurny et al. (2017) used exactly this method (for most fireballs). If no 
> fragmentation is considered, it is identical to the Ceplecha et al. (1993) 
> ablation model. So, please, reformulate parts of paragraphs 3 and 4.

Thank you for the insightful details, the suggestions are incorporated in the paper.

> The other corrections are just typos:
> Page 10, line 49: … between the asteroidal type A and cometary type C (not B).
> Page 12, line 53: stream (not steam)

Corrected.


> References: The accent in Spurny, Shrbeny is incorrect. It is \’ (as in 
> Korlevic), not \`. The same is for Pokorny (in Abedin et al. 2017, 2018).
> The reference Spurny et al. (2017) is incomplete.

Corrected.
